A characterization of D-norms and their generators based on the family of spectral functions

Aulbach et al. (2012) introduced the concept of D-norms in the framework of functional extreme value theory (EVT) extending the multivariate case in a natural manner. In particular, the distribution of a standard max-stable process (MSP) {\eta} \in C[0,1] is completely determined by its functional distribution function, which itself is given by some D-norm. In order to generate a generalized Pareto process (GPP) that is in the functional domain of attraction of {\eta}, one may use the fact that every D-norm is defined by some generator process with continuous sample paths. It is, however, still unknown which generator must be chosen such that a given D-norm arises. This is the content of the present paper. We will, moreover, show that a generator process may be decomposed into a functional deterministic part and a univariate random one.

==> abbr.tex <==
\newcommand{\Rstat}{\textsc{R}\xspace}
\newcommand{\Mathematica}{\textsc{Mathematica}\xspace}

\newcommand{\eur}{\euro\xspace}

\newcommand{\iid}{i.\,i.\,d.\xspace}


% English
\newcommand{\eg}{e.\,g.,\xspace}
\newcommand{\ie}{i.\,e.,\xspace}
\newcommand{\as}{a.\,s.\xspace}

% German
\AtBeginDocument{\renewcommand{\dh}{d.\,h.\xspace}}
    % um Konflikte mit dem hyperref-Paket zu vermeiden (\dh ist urspr\"{u}nglich ein
    % Sonderzeichen, das nicht in allen Font-Kodierungen verf\"{u}gbar ist.)
\newcommand{\Dh}{D.\,h.\xspace}
\newcommand{\zB}{z.\,B.\xspace}
\newcommand{\fs}{f.\,s.\xspace}
\newcommand{\iA}{i.\,A.\xspace}
\newcommand{\idR}{i.\,d.\,R.\xspace}
\newcommand{\ua}{u.\,a.\xspace}
\newcommand{\uU}{u.\,U.\xspace}
\newcommand{\oBdA}{o.B.d.A.\xspace}
\newcommand{\OBdA}{O.B.d.A.\xspace}

\newcommand{\gq}[1]{\glq#1\grq}
\newcommand{\gqq}[1]{\glqq#1\grqq}
\newcommand{\eq}[1]{`#1'}
\newcommand{\eqq}[1]{``#1''}


==> mathdefs.tex <==
% Klammern
\makeatletter
    \newcommand{\paren}{\@ifstar{\paren@Star}{\paren@NoStar}}
        \@DeclarePairedDelimiterXY{paren@Star}{2}{(}{)}{#1 \mathrel{}\mathclose{}\delimsize|\mathopen{}\mathrel{} #2}
        \@DeclarePairedDelimiterY{paren@NoStar}{(}{)}
    \@DeclarePairedDelimiterY{brac}{[}{]}
    \newcommand{\set}{\@ifstar{\set@Star}{\set@NoStar}}
        \@DeclarePairedDelimiterXY{set@Star}{2}{\{}{\}}{#1 \mathrel{}\mathclose{}\delimsize|\mathopen{}\mathrel{} #2}
        \@DeclarePairedDelimiterY{set@NoStar}{\{}{\}}
    \newcommand{\curly}[2][]{\set@NoStar[#1]{#2}}
\makeatother

% Intervalle
\makeatletter
    \@DeclarePairedDelimiterXY{intoo}{2}{(}{)}{#1,#2}
    \@DeclarePairedDelimiterXY{intcc}{2}{[}{]}{#1,#2}
    \@DeclarePairedDelimiterXY{intoc}{2}{(}{]}{#1,#2}
    \@DeclarePairedDelimiterXY{intco}{2}{[}{)}{#1,#2}
\makeatother

% Folgen, Familien, Prozesse u. \"{a}.
\makeatletter
    \newcommand{\coll}{\@ifstar{\coll@Star}{\coll@NoStar}}
        \newcommand{\coll@Star}[4][]{{\paren[#1]{#2}}_{#3\in #4}}
        \newcommand{\coll@NoStar}[4][]{%
            \@ifMacroDefined{\expandafter\csname\removebs#2sub\endcsname}{%
                {\paren[#1]{\expandafter\csname\removebs#2sub\endcsname{#3}}}_{#3\in #4}%
            }{%
                {\paren[#1]{#2_#3}}_{#3\in #4}
            }
        }
    \newcommand{\pro}{\coll}
    \newcommand{\seq}{\@ifstar{\seq@Star}{\seq@NoStar}}
        \newcommand{\seq@Star}[3][\N]{\coll@Star{#2}{#3}{#1}}
        \newcommand{\seq@NoStar}[3][\N]{\coll@NoStar{#2}{#3}{#1}}
    \newcommand{\ocoll}{\@ifstar{\coll@Star}{\ocoll@NoStar}}
        \newcommand{\ocoll@NoStar}[4][]{\coll@Star[#1]{{#2}_{#3}}{#3}{#4}}
    \newcommand{\opro}{\ocoll}
    \newcommand{\oseq}{\@ifstar{\oseq@Star}{\oseq@NoStar}}
        \newcommand{\oseq@Star}[3][\N]{\ocoll@Star{#2}{#3}{#1}}
        \newcommand{\oseq@NoStar}[3][\N]{\ocoll@NoStar{#2}{#3}{#1}}
\makeatother

% Grundr\"{a}ume
\makeatletter
    \newcommand{\unit}{\@ifstar{\unit@Star}{\unit@NoStar}}
        \newcommand{\unit@Star}{\intoo{0}{1}}
        \newcommand{\unit@NoStar}{\intcc{0}{1}}
    \newcommand{\Runit}{{\R^{\unit}}}
    \@DeclareFunctionSpace[mathcal]{C}{unit} % \Cspace \Cplus \Cbarplus \Cmin \Cbarmin; \Cspace[\intcc{a}{b}] \Cspace* \Cspace*[X] \Cspace*[X][big] etc.
    \@DeclareFunctionSpace[mathcal]{D}{unit}
    \@DeclareFunctionSpace[mathcal]{E}{unit}
\makeatother
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Rbar}{\closure{\R}}

% Mengensysteme (\sigma-Algebren, Topologien etc.)
\makeatletter
    \newcommand{\compl}{\@ifstar{\compl@Star}{\compl@NoStar}}
        \newcommand{\compl@Star}[2][]{{\paren[#1]{#2}^{\mathrm{c}}}}
        \newcommand{\compl@NoStar}[1]{{#1^{\mathrm{c}}}}
    \newcommand{\inducedtop}{\@ifstar{\inducedtop@Star}{\inducedtop@NoStar}}
        \newcommand{\inducedtop@Star}[3][]{\sups{#2}{-1}\paren[#1]{#3}}
        \newcommand{\inducedtop@NoStar}[2][]{\Tau[#1]{#2}}
        \@DeclareMathOperator*{Tau}{\tau}
    \newcommand{\inducedsig}{\@ifstar{\inducedtop@Star}{\inducedsig@NoStar}}
        \newcommand{\inducedsig@NoStar}[2][]{\sigma\paren[#1]{#2}}
    \newcommand\cart\bigtimes
    \let\prodtop\bigotimes
    \let\prodsig\prodtop
    \let\prodspace\prod
    \newcommand{\powerset}[1]{\@powerset\paren{#1}}
        \DeclareMathOperator{\@powerset}{\mathcal{P}}
    \newcommand{\ball}{\@ifstar{\ball@Star}{\ball@NoStar}}
        \newcommand{\ball@Star}[4][]{\@ball_{#2}\paren[#1]{#3,#4}}
        \newcommand{\ball@NoStar}[3][]{\@ball\paren[#1]{#2,#3}}
        \DeclareMathOperator{\@ball}{\textit{B}}
\makeatother
\newcommand{\B}{\mathbb{B}}
\newcommand{\Bunit}{\B_{\unit}}
\newcommand{\BunitC}{\Bunit^{C}}
\makeatletter
    \@DeclareFunction*[mathcal]{spectraldens}{G}
\makeatother
\newcommand{\sA}{\mathcal{A}}
\newcommand{\sB}{\mathcal{B}}
\newcommand{\sC}{\mathcal{C}}
\newcommand{\sH}{\mathcal{H}}
\newcommand{\sS}{\mathcal{S}}

% Topologie im Besonderen
\makeatletter
    \newcommand{\opensets}{\@ifstar{\opensets@Star}{\opensets@NoStar}}
        \newcommand{\opensets@Star}{\mathcal{H}}
        \newcommand{\opensets@NoStar}{\mathcal{G}}
    \newcommand{\base}{\@ifstar{\base@Star}{\base@NoStar}}
        \newcommand{\base@Star}[2][]{\base@NoStar\paren[#1]{#2}}
        \newcommand{\base@NoStar}{\mathcal{B}}
    \newcommand{\subbase}{\@ifstar{\subbase@Star}{\subbase@NoStar}}
        \newcommand{\subbase@Star}[2][]{\subbase@NoStar\paren[#1]{#2}}
        \newcommand{\subbase@NoStar}{\underline{\mathcal{B}}}
\makeatother
\newcommand{\closedsets}{\mathcal{F}}
\newcommand{\compactsets}{\mathcal{K}}
\makeatletter
    \newcommand{\interior}{\@ifstar{\interior@Star}{\interior@NoStar}}
        \newcommand{\interior@Star}[2][]{{\widering{#2}}}
        \newcommand{\interior@NoStar}[1]{{\mathring{#1}}}
    \newcommand{\closure}{\@ifstar{\closure@Star}{\closure@NoStar}}
        \newcommand{\closure@Star}[1]{\overline{#1}}
        \newcommand{\closure@NoStar}[1]{\widebar{#1}}
    \newcommand{\frontier}{\@ifstar{\frontier@Star}{\frontier@NoStar}}
        \newcommand{\frontier@Star}[2][]{\Partial[#1]{#2}}
        \newcommand{\frontier@NoStar}[1]{\Partial*{#1}}
        \@DeclareMathOperator*{Partial}{\partial\mspace{-1mu}}
\makeatother

% Operatoren
\makeatletter
    \let\P\undefined \@DeclareMathOperator{P}
    \@DeclareMathOperator{E}
    \@DeclareMathOperator{Var}
    \@DeclareMathOperator{Cov}
    \@DeclareMathOperator{Cor}
    \@DeclareMathOperator{diag}
    \newcommand*{\supp}[2][]{\operatorname{\mathrm{supp}}\paren[#1]{\mathord{#2}}}
    \newcommand*{\im}{\@ifstar{\im@Star}{\im@NoStar}}
        \newcommand*{\im@Star}[3][]{\operatorname{#2}\paren[#1]{#3}}
        \newcommand*{\im@NoStar}[2][]{\operatorname{\mathrm{Im}}\paren[#1]{\mathord{#2}}}
    \AtBeginDocument{
        \let\O\undefined \@DeclareMathOperator*[mathcal]{O}{O}
        \let\o\undefined \@DeclareMathOperator*[textit]{o}{o}
    }
\makeatother

% Funktionen und Zufallsgr\"{o}{\ss}en
\makeatletter
    \let\exp\undefined \@DeclareFunction*{exp}{exp}
    \let\log\undefined \@DeclareFunction*{log}{log}
    \let\sin\undefined \@DeclareFunction*{sin}{sin}
    \let\arcsin\undefined \@DeclareFunction*{arcsin}{arcsin}
    \@DeclareFunction*{C}{C}
    \let\Finv\undefined \@DeclareFunction*{F}{F}
    \@DeclareFunction*{G}{G}
    \@DeclareFunction*{W}{W}
    \@DeclareFunction{U}
    \@DeclareFunction{X}
    \@DeclareFunction{Y}
    \@DeclareFunction{f}
    \@DeclareFunction{g}
    \@DeclareFunction{h}
    \newcommand{\ind}{\@ifstar{\ind@Star}{\ind@NoStar}}
        \newcommand{\ind@Star}[2]{\@indsub*{#1}{#2}}
        \newcommand{\ind@NoStar}[1]{\@indsub{#1}}
        \@DeclareFunction*{@ind}{\ensuremath{\mathds{1}}}
    \@DeclareFunction*[]{proj}{\pi}
\makeatother
\newcommand\rest[2]{{% we make the whole thing an ordinary symbol
    \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
    #1 % the function
    \vphantom{\big|} % pretend it's a little taller at normal size
    \right|_{#2} % this is the delimiter
}} % Quelle: http://tex.stackexchange.com/a/22255

% Ma{\ss}e und Verteilungen
\makeatletter
    \newcommand{\Ud}{\@ifstar{\Ud@Star}{\Ud@NoStar}}
        \newcommand{\Ud@Star}[2][]{\@Ud\paren[#1]{#2}}
        \newcommand{\Ud@NoStar}[1][\unit]{\mathcal{U}{#1}}
        \DeclareMathOperator{\@Ud}{\mathcal{U}}
    \newcommand{\Nd}{\@ifstar{\Nd@Star}{\Nd@NoStar}}
        \newcommand{\Nd@Star}[3][]{\@Nd\paren[#1]{#2,#3}}
        \newcommand{\Nd@NoStar}[1][]{\Nd@Star[#1]{0}{1}}
        \DeclareMathOperator{\@Nd}{\mathcal{N}}
    \newcommand{\distr}{\@ifstar{\distr@Star}{\distr@NoStar}}
        \newcommand{\distr@Star}[2][]{\@L\paren[#1]{#2}}
        \newcommand{\distr@NoStar}[2][\@P]{{#1}\ast{#2}}
        \DeclareMathOperator{\@L}{\mathcal{L}}
%    \newcommand{\distrP}[3][][\@P]{\paren[#1]{\dist@NoStar[#2]{#3}}}
\makeatother

% Integration
\makeatletter
    \newcommand{\intdif}{\@ifstar{\intdif@Star}{\intdif@NoStar}}
        \newcommand{\intdif@Star}[5][]{\int_{#2}^{#1} #3 \mspace{1mu}#4\paren{\dif #5}}
        \newcommand{\intdif@NoStar}[4][]{\int_{#2}^{#1} #3 \dif #4}
        \DeclareMathOperator{\dif}{d\mspace{-3mu}}
\makeatother

% Normen und Metriken
\makeatletter
    \@DeclarePairedDelimiterY{abs}{\lvert}{\rvert}
    \@DeclarePairedDelimiterY{norm}{\lVert}{\rVert}
    \newcommand{\normd}{\norm{{\cdot}}}
    \newcommand{\pnorm}{\@ifstar{\pnorm@Star}{\pnorm@NoStar}}
        \newcommand{\pnorm@Star}[4][]{{\norm[#1]{#2}_{#3,#4}}}
        \newcommand{\pnorm@NoStar}[3][]{{\norm[#1]{#2}_{#3}}}
    \newcommand{\pnormd}{\@ifstar{\pnormd@Star}{\pnormd@NoStar}}
        \newcommand{\pnormd@Star}[2]{\pnorm*{{\cdot}}{#1}{#2}}
        \newcommand{\pnormd@NoStar}[1]{\pnorm{{\cdot}}{#1}}
    \newcommand{\pnorme}{\@ifstar{\pnorme@Star}{\pnorme@NoStar}}
        \newcommand{\pnorme@Star}[5][]{{\norm[#1]{#2}_{#3,#4}^{#5}}}
        \newcommand{\pnorme@NoStar}[4][]{{\norm[#1]{#2}_{#3}^{#4}}}
    \newcommand{\supnorm}[2][]{\pnorm[#1]{#2}{\infty}}
    \newcommand{\supnormd}{\supnorm{{\cdot}}}
    \newcommand{\supnorme}[3][]{\pnorme[#1]{#2}{\infty}{#3}}
    \newcommand{\dnorm}{\@ifstar{\dnorm@Star}{\dnorm@NoStar}}
        \newcommand{\dnorm@Star}[3][]{\pnorm*[#1]{#2}{D}{#3}}
        \newcommand{\dnorm@NoStar}[2][]{\pnorm[#1]{#2}{D}}
    \newcommand{\dnormd}{\@ifstar{\dnormd@Star}{\dnormd@NoStar}}
        \newcommand{\dnormd@Star}[1]{\dnorm*{{\cdot}}{#1}}
        \newcommand{\dnormd@NoStar}{\dnorm{{\cdot}}}
    \newcommand{\dnorme}{\@ifstar{\dnorme@Star}{\dnorme@NoStar}}
        \newcommand{\dnorme@Star}[4][]{{\pnorme*[#1]{#2}{D}{#3}^{#4}}}
        \newcommand{\dnorme@NoStar}[3][]{{\pnorme[#1]{#2}{D}^{#3}}}
    \newcommand{\metric}{\@ifstar{\metric@Star}{\metric@NoStar}}
        \newcommand{\metric@Star}[4][]{\metricd@Star{#2}\paren[#1]{#3,#4}}
        \newcommand{\metric@NoStar}[3][]{\@metric\paren[#1]{#2,#3}}
        \DeclareMathOperator{\@metric}{\textit{d}}
    \newcommand{\metricd}{\@ifstar{\metricd@Star}{\metricd@NoStar}}
        \newcommand{\metricd@Star}[1]{\@metric_{#1}}
        \newcommand{\metricd@NoStar}{\@metric{}}
\makeatother

% Symbole
\newcommand{\eps}{\varepsilon}
\newcommand{\bfzero}{\bm{0}}
\newcommand{\bfone}{\bm{1}}
\newcommand{\bfinfty}{\bm{\infty}}

% Fett-Buchstaben
\makeatletter
    \@DeclareBM{A}
    \@DeclareBM{B}
    \@DeclareBM{C}
    \@DeclareBM{D}
    \@DeclareBM{E}
    \@DeclareBM{F}
    \@DeclareBM{G}
    \@DeclareBM{H}
    \@DeclareBM{I}
    \@DeclareBM{J}
    \@DeclareBM{K}
    \@DeclareBM{L}
    \@DeclareBM{M}
    \@DeclareBM{N}
    \@DeclareBM{O}
    \@DeclareBM{P}
    \@DeclareBM{Q}
    \@DeclareBM{R}
    \@DeclareBM{S}
    \@DeclareBM{T}
    \@DeclareBM{U}
    \@DeclareBM{V}
    \@DeclareBM{W}
    \@DeclareBM{X}
    \@DeclareBM{Y}
    \@DeclareBM{Z}
    \@DeclareBM{a}
    \@DeclareBM{b}
    \@DeclareBM{c}
    \@DeclareBM{d}
    \@DeclareBM{e}
    \@DeclareBM{f}
    \@DeclareBM{g}
    \@DeclareBM{h}
    \@DeclareBM{i}
    \@DeclareBM{j}
    \@DeclareBM{k}
    \@DeclareBM{l}
    \@DeclareBM{m}
    \@DeclareBM{n}
    \@DeclareBM{o}
    \@DeclareBM{p}
    \@DeclareBM{q}
    \@DeclareBM{r}
    \@DeclareBM{s}
    \@DeclareBM{t}
    \@DeclareBM{u}
    \@DeclareBM{v}
    \@DeclareBM{w}
    \@DeclareBM{x}
    \@DeclareBM{y}
    \@DeclareBM{z}
    \@DeclareBM*{Lambda}
    \@DeclareBM*{Sigma}
    \@DeclareBM*{alpha}
    \@DeclareBM*{beta}
    \@DeclareBM*{chi}
    \@DeclareBM*{eps}
    \@DeclareBM*{eta}
    \@DeclareBM*{gamma}
    \@DeclareBM*{lambda}
    \@DeclareBM*{mu}
    \@DeclareBM*{omega}
    \@DeclareBM*{sigma}
    \@DeclareBM*{xi}
    \@DeclareBM*{zeta}
\makeatother


==> refnames_en.tex <==
\newcommand{\paname}{\partname}
\newcommand{\chapname}{\chaptername}
\newcommand{\secname}{Section}
\newcommand{\subname}{Section}

\newcommand{\defnname}{Definition}
\newcommand{\examname}{Example}
\newcommand{\lemname}{Lemma}
\newcommand{\theoname}{Theorem}
\newcommand{\propname}{Proposition}
\newcommand{\corname}{Corollary}
\newcommand{\remname}{Remark}
\newcommand{\itemname}{part}

\newcommand{\eqnname}{Equation}
\newcommand{\figname}{\figurename}
\newcommand{\tblname}{\tablename}
\newcommand{\footnotename}{Footnote}

\newcommand{\exname}{Exercise}
\newcommand{\solname}{Solution}


==> refs.tex <==
\newrefformat{pa}{{\paname\,\ref{#1}}}
\newrefformat{chap}{{\chapname\,\ref{#1}}}
\newrefformat{sec}{{\secname\,\ref{#1}}}
\newrefformat{sub}{\subname \emph{\nameref{#1}}}  % Der \nameref-Befehl wird vom hyperref-Paket zur Verf\"{u}gung gestellt

\newrefformat{defn}{{\defnname\,\ref{#1}}}
\newrefformat{exam}{{\examname\,\ref{#1}}}
\newrefformat{lem}{{\lemname\,\ref{#1}}}
\newrefformat{theo}{{\theoname\,\ref{#1}}}
\newrefformat{prop}{{\propname\,\ref{#1}}}
\newrefformat{cor}{{\corname\,\ref{#1}}}
\newrefformat{rem}{{\remname\,\ref{#1}}}
\newrefformat{item}{{\itemname\,\eqref{#1}}}

\newrefformat{eqn}{{\eqnname\,\eqref{#1}}}
\newrefformat{fig}{{\figname\,\ref{#1}}}
\newrefformat{tbl}{{\tblname\,\ref{#1}}}
\newrefformat{footnote}{{\footnotename\,\ref{#1}}}

\newrefformat{ex}{{\exname\,\ref{#1}}}


==> thms.tex <==
\theoremstyle{defn}
    \@ifpackagewith{\CurrentPackage}{eqn}{
        \newtheorem{definition}[\theoremcounter]{\defnname}
    }{
        \newtheorem{definition}{\defnname}[section]
    }
    \newtheorem{example}[\theoremcounter]{\examname}
\theoremstyle{theo}
    \newtheorem{lemma}[\theoremcounter]{\lemname}
    \newtheorem{theorem}[\theoremcounter]{\theoname}
    \newtheorem{proposition}[\theoremcounter]{\propname}
    \newtheorem{corollary}[\theoremcounter]{\corname}
\theoremstyle{rem}
    \newtheorem{remark}[\theoremcounter]{\remname}

